A Simple Rewrite System for the Normalization of Linear Temporal Logic

In the mid 80s, Lichtenstein, Pnueli, and Zuck showed that every formula of Past LTL (the extension of Linear Temporal Logic with past operators) is equivalent to a conjunction of formulas of the form $\mathbf{G}\mathbf{F} \varphi \vee \mathbf{F}\mathbf{G} \psi$, where $\varphi$ and $\psi$ contain only past operators. Some years later, Chang, Manna, and Pnueli derived a similar normal form for LTL. Both normalization procedures have a non-elementary worst-case blow-up, and follow an involved path from formulas to counter-free automata to star-free regular expressions and back to formulas. In 2020, Sickert and Esparza presented a direct and purely syntactic normalization procedure for LTL yielding a normal form similar to the one by Chang, Manna, and Pnueli, with a single exponential blow-up, and applied it to the problem of constructing a succinct deterministic $\omega$-automaton for a given formula. However, their procedure had exponential time complexity in the best case. In particular, it does not perform better for formulas that are almost in normal form. In this paper we present an alternative normalization procedure based on a simple set of rewrite rules.

==> Sections/easyproof.tex <==
\section{The Normalization Theorem}
\label{sec:overview}

\begin{definition}
\label{def:normalform}
A formula of LTL is in \emph{normal form} if it is a positive Boolean combination of formulas of 
$\Sigma_2$ and formulas of the form $\G\F \varphi$, where $\varphi \in \Sigma_1$ (and so $\G\F \varphi \in \Pi_2$). 
\end{definition}

We prove that every formula of L(\U, \W, \X) can be normalized.  A formula of 
L(\U, \W, \X) is a \emph{temporal formula} if the operator at the top of its syntax tree is
$\U$, $\W$, or $\X$.  The following fact is an imediate consequence of the definition:

\begin{factt}
\label{fact:Bool}
If all temporal formulas are normalizable, then all formulas are normalizable. 
\end{factt}

%\paragraph{Disjunctive-Conjunctive-Normalform.} Because of the identities
%$$
%\begin{array}{cc}
%(\varphi_1 \wedge \varphi_2) \Z \varphi_3 \equiv (\varphi_1 \Z \varphi_3) \wedge (\varphi_2 \Z \varphi_3) \\
%\varphi_1 \Z (\varphi_2 \vee \varphi_3 ) \equiv (\varphi_1 \Z \varphi_2) \vee (\varphi_1 \Z \varphi_3) \\
%\end{array}
%$$
%it suffices to prove the result for formulas of $L(\U, \W)$ with syntax
%$$\varphi ::=  a \mid  \left( \vee \varphi \right) \U \left( \wedge \varphi \right) \mid \left( \vee \varphi \right) \W \left( \wedge \varphi \right)$$

\subsection{$\G\F\Sigma_2$-formulas can be normalized}

The key to the normalization theorem is to observe that formulas of the form $\G\F\varphi$ satisy very special properties.

We consider formulas $\varphi$ with a ``hole'' that can be filled with a formula. 
Formally, let $\hole$ be a symbol denoting a special atomic proposition. A formula with a hole is a formula with one
single occurrence of $\hole$. We let $\varphi\hole$ denote that $\varphi$ is a formula with a hole, and denote by $\varphi[\psi]$ the result of filling the hole with $\psi$; formally, $\varphi[\psi]$ is the result of substituting $\psi$ for the unique occurrence of $\hole$ in $\varphi$. For example, if $\varphi\hole = a \W \hole$, then $\varphi[a \U c ] = a \W (a \U c)$ and $\varphi[\X b ] = a \W \X b$.

\begin{lemma}
\label{lem:GF}
For every formula $\varphi[\psi_1 \W \psi_2]$:
$$\G\F \varphi [\psi_1 \W \psi_2] \equiv (\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]) \vee  (\F\G \psi_1 \wedge \G\F \varphi [\true]) \vee \G\F \varphi [\false]$$
\end{lemma}
\begin{proof}
The proof repeatedly uses the following observation, an immediate consequence of the fact that $\varphi$ is in negation normal form:

\begin{equation}
\text{For every two formulas $\psi, \psi'$, if $\psi \models \psi'$ then  $\varphi [\psi] \models \varphi [\psi']$.} \label{sta}
\end{equation}

\noindent ($\leftmodels$)  We prove the following three claims, which immediately imply the result:
\begin{itemize}
\item $\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]  \models  \G\F \varphi [\psi_1 \W \psi_2]$. \\
Follows from $\psi_1 \U \psi_2 \models \psi_1 \W \psi_2$ and (\ref{sta}).
\item $\F\G \psi_1 \wedge \G\F \varphi [\true] \models \G\F \varphi [\psi_1 \W \psi_2]$. \\
Assume $w \models \F\G \psi_1 \wedge \G\F \varphi [\true]$. Then  infinitely many suffixes of $w$ satisfy $\G\psi_1$ and so $\varphi [\psi_1 \W \psi_2]$. These suffixes also satisfy $\psi_1 \W \psi_2$, and we are done.
\item $\G\F \varphi [\false] \models \G\F \varphi [\psi_1 \W \psi_2]$.\\
Follows from $\false \models \psi_1 \W \psi_2$ and (\ref{sta}).
\end{itemize}

\medskip

\noindent ($\models$)  Assume $w$ satisfies $\G\F \varphi [\psi_1 \W \psi_2]$, and so that  $w' \models \varphi [\psi_1 \W \psi_2]$ for infinitely many suffixes $w'$ of $w$. We prove the following three claims, which immediately imply the result:
\begin{itemize}
\item If $w \models \G\F \psi_2$ then  $w \models \G\F \varphi [\psi_1 \U \psi_2]$. \\
Since $w \models \G\F \varphi [\psi_1 \W \psi_2]$, it suffices to show that the infinitely many suffixes $w'$ of $w$ satisfying $\varphi [\psi_1 \W \psi_2]$ also satisfy $\varphi [\psi_1 \U \psi_2]$. 
For this, observe that  $w' \models \psi_1 \W \psi_2$ and  $w \models \G\F \psi_2$ imply $w' \models \psi_1 \U \psi_2$. 

\item If $w \models \F\G \psi_1$ then $w \models \G\F \varphi [\true]$.\\
Since $w \models \F\G \psi_1 \wedge \G\F \varphi [\psi_1 \W \psi_2]$, infinitely many suffixes of $w$ satisfy $\G\psi_1$ and $\varphi [\psi_1 \W \psi_2]$. Since $\G\psi_1 \models \psi_1 \W \psi_2$, these suffixes also satisfy $\psi_1 \W \psi_2$, and so also $\varphi [\true]$.

\item If $w \not\models \G\F \psi_2$ and $w \not\models \F\G \psi_1$, then $w \models \G\F \varphi [\false]$. \\
Since $w \not\models \G\F \psi_2$ and $w \not\models \F\G \psi_1$, 
infinitely many suffixes of $w$ satisfying $\varphi [\psi_1 \W \psi_2]$ do not satisfy $\psi_1 \W \psi_2$.
So they satisfy $\varphi [\false]$, which implies $w \models \G\F \varphi [\false]$.
\end{itemize}
\end{proof}

\begin{proposition}
\label{prop1}
Formulas of $\G\F \Sigma_2$ can be normalized.
\end{proposition}
\begin{proof}
Let $\G\F \varphi \in \G\F \Sigma_2$.  We prove that $\G\F \varphi$ can be normalized by induction on the number of \W-subformulas of $\varphi$. If there are none, then $\G\F\varphi \in \G\F\Pi_1$ and we are done. Otherwise, let $\psi_1 \W \psi_2$ be a  \W-subformula of $\varphi$. By Lemma \ref{lem:GF} we have
$$\G\F \varphi [\psi_1 \W \psi_2] \equiv (\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]) \vee  (\F\G \psi_1 \wedge \G\F \varphi [\true]) \vee \G\F \varphi [\false]$$
By induction hypothesis $\G\F \psi_2$, $\G\F \varphi [\psi_1 \U \psi_2]$, $\G\F\varphi [\true]$, and $\G\F \varphi [\false]$ can be normalized. Further, since $\varphi \in \Sigma_2$ we have $\psi_1 \in \Pi_1$ and $\F\G \psi_1 \in \Sigma_2$. So $\F\G \psi_1$ is also in normal form, and we are done.
\end{proof}

\subsection{L(\U, \G\F) can be normalized}

\begin{definition}
\label{prop:boolup}
$Cl(\Sigma_2; \U, \G\F)$ denotes the closure of $\Sigma_2$ under $\U$ and $\G\F$, i.e., the smallest set of formulas ${\cal F}$ satisfying: 
\begin{itemize}
\item $\Sigma_2 \subseteq {\cal F}$; 
\item if $\varphi, \psi \in {\cal F}$, then $\varphi \U \psi \in {\cal F}$; and
\item if $\varphi \in {\cal F}$, then $\G\F \varphi \in {\cal F}$.
\end{itemize}
\end{definition}

\begin{proposition}
\label{prop:boolup}
Formulas of $Cl(\Sigma_2; \U, \G\F)$ can be normalized.
\end{proposition}
\begin{proof}
Let $\varphi$ be a formula of $Cl(\Sigma_2; \U, \G\F)$. We show that $\varphi$ is equivalent to a Boolean combination
of formulas of $\Sigma_2$ and formulas of $\G\F \Sigma_2$. The result then follows from Proposition \ref{prop1}.

Let $\varphi'$ be the result of exhaustively applying the following equivalences to $\varphi$ (from left to right):

\begin{eqnarray}
(\psi_1 \wedge \psi_2) \U \psi_3 & \equiv & \psi_1 \U \psi_3 \wedge \psi_2 \U \psi_3 \label{id1}\\
\psi_1 \U (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \U \psi_2 \vee \psi_1 \U \psi_3 \label{id2}\\
(\psi_1 \vee \G\F \psi) \,\U \psi_2 & \equiv  & (\G\F \psi \wedge  \psi_2) \vee \psi_1 \U \psi_2  \label{id3}\\
\psi_1  \,\U (\G\F \psi \wedge \psi_2) & \equiv  &\G\F \psi \wedge  \psi_1 \U \varphi_2 \label{id4} \\
\G\F( \psi_1 \wedge \G\F \psi_2) &\equiv & \G\F \psi_1 \wedge \G\F \psi_2  \label{id1p}\\
\G\F( \psi_1 \vee \G\F \psi_2) &\equiv & \G\F \psi_1 \vee \G\F \psi_2  \label{id2p}\\
\G\F( \G\F\varphi) &\equiv & \G\F \varphi \label{id3p}
\end{eqnarray}

By (\ref{id1})-(\ref{id4}), no path of the syntax tree of $\varphi'$ contains a \U{} before a \G\F. By (\ref{id1p})-(\ref{id3p}),
no path of the tree contains two or more occurrences of \G\F. So the projection of every path of the syntax tree onto
\G\F, \U, and \W{} belongs to the regular expression $(\epsilon + \G\F) \U^*\W^*$. So $\varphi'$ is a Boolean combination of formulas of $\Sigma_2$ and formulas of $\G\F \Sigma_2$.

%The proof is by structural induction. By Fact \ref{fact:Bool} it
%suffices to consider two cases:
%
%\medskip
%
%\noindent Case 1: $\varphi = \G\F \varphi_1$. \\
%By induction hypothesis, $\varphi_1$ can be normalized, i.e., we can assume it is a positive Boolean combination of 
%formulas of $\Sigma_2$ and $\G\F\Sigma_1$, and w.l.o.g. that it is in disjunctive normal form. 
%We proceed by induction on the number $k$ of disjuncts of $\varphi_1$. 
%
%\medskip \noindent Base: $k=1$. Then $\varphi_1$ is a conjunction. We proceed by induction on the number of conjuncts that are formulas of $\G\F\Sigma_1$. If there are none, then $\varphi_1 \in \Sigma_2$ and the result follows from Proposition \ref{prop1}. If there is at east one, then 
%$\varphi_1 = \varphi_2 \wedge \G\F \varphi_3$ for some $\varphi_3 \in \Pi_1$. We apply
%$$\G\F \varphi_1 \equiv \G\F( \varphi_2 \wedge \G\F \varphi_3) \equiv \G\F \varphi_2 \wedge \G\F \varphi_3 \  .$$
%\noindent By induction hypothesis (induction on $\ell$), $\G\F \varphi_2$ can be normalized, and $\G\F \varphi_3$ is already in normal form, because $\varphi_3 \in \Pi_1$. So $\G\F \varphi_1$ can be normalized.
%
%\medskip \noindent Step: $k>1$. Then $\varphi_1 = \varphi_2 \vee \varphi_3$  for some formulas $\varphi_2, \varphi_3$.
%Since $\G\F (\varphi_2 \vee \varphi_3) \equiv \G\F \varphi_2 \vee \G\F \varphi_3$, by induction hypothesis (induction on $k$) the formulas $\G\F \varphi_2$ and $\G\F \varphi_3$ can be normalized, and we are done. 
%
%\bigskip\noindent Case 2: $\varphi = \varphi_1 \U \varphi_2$. By induction hypothesis, $\varphi_1$ and $\varphi_2$ can be normalized, i.e., we can assumethey are positive Boolean combinations of formulas of $\Sigma_2$ and $\G\F\Sigma_1$. By exhaustively applying the identities 
%\begin{eqnarray}
%(\psi_1 \wedge \psi_2) \U \psi_3 & \equiv & \psi_1 \U \psi_3 \wedge \psi_2 \U \psi_3 \label{id1}\\
%\psi_1 \U (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \U \psi_2 \vee \psi_1 \U \psi_3 \label{id2}\\
%(\psi_1 \vee \G\F \psi) \,\U \psi_2 & \equiv  & (\G\F \psi \wedge  \psi_2) \vee \psi_1 \U \psi_2  \label{id3}\\
%\psi_1  \,\U (\G\F \psi \wedge \psi_2) & \equiv  &\G\F \psi \wedge  \psi_1 \U \varphi_2 \label{id4}
%\end{eqnarray}
%\noindent which allow to move $\G\F$ up across $\U$, we obtain that $\varphi$ is equivalent to a positive Boolean combination of formulas of $\G\F\Sigma_1$ and formulas of the form $\psi_1 \U \psi_2$, where $\psi_1$ and $\psi_2$ have no $\G\F$-subformulas.  But then $\psi_1 \U \psi_2 \in \Sigma_1$, and we are done. 
\end{proof}

\subsection{$\Sigma_2 \W \Sigma_2$ can be normalized}
\begin{proposition} 
\label{prop:s2ws2}
Formulas of $\Sigma_2 \W \Sigma_2$ can be normalized.
\end{proposition}
\begin{proof}
Let $\varphi_1 \W \varphi_2$ be a formula of $\Sigma_2 \W \Sigma_2$. 
We proceed by induction on the total number of \U-subformulas of $\varphi_1$ and $\varphi_2$.
Consider three cases:

\begin{itemize}
\item Neither $\varphi_1$ nor $\varphi_2$ have \U-subformulas.\\
Then $\varphi_1 \W \varphi_2 \in \Pi_1$, and so in particular it is in normal form.

\item $\varphi_2$ has at least one \U-subformula. \\
Assume w.l.o.g. that $\varphi_2$ is in disjunctive normal form. 
We proceed by induction on the number $k$ of disjuncts of $\varphi_2$. 

\smallskip\noindent If $k=1$ then $\varphi_2 = (\psi_1 \U \psi_2 \wedge \psi_3)$ for formulas $\psi_1, \psi_2,\psi_3 \in \Sigma_2$
(indeed, since $\varphi_2$ has at least one \U-subformula, then at least one of its conjuncts has one, and the top operator of that conjunct, which must be a temporal operator, is \U{}, because otherwise $\varphi_2 \notin \Sigma_2$). 
Then we have 

%Observe that the total number of \U-subformulas of $\psi_1, \psi_2,\psi_3$ is one less than the total number of  $\varphi_1$ and $\varphi_2$. We have:

$$\varphi_1 \W \varphi_2 
\equiv   \varphi_1 \W (\psi_1 \U \psi_2 \wedge \psi_3) 
\equiv   \varphi_1 \U  (\psi_1 \U \psi_2 \wedge \psi_3) \vee  \G \varphi_1
$$
Since $\psi_1, \psi_2,\psi_3 \in \Sigma_2$,  we have $\varphi_1 \U  (\psi_1 \U \psi_2 \wedge \psi_3) \in \Sigma_2$, and so in normal form.  Since the number of \U-subformulas of $\G \varphi_1$ is strictly smaller than that of $\varphi_1 \W \varphi_2$, by induction hypothesis $\G \varphi_1$ can be normalized too.

\smallskip\noindent If $k > 1$ then $\varphi_2 = \varphi_{21} \vee \varphi_{22}$. So $\varphi_1 \W \varphi_2 \equiv \varphi_1 \W \varphi_{21} \vee \varphi_1 \W \varphi_{22}$. By induction hypothesis (induction on $k$), both $\varphi_1 \W \varphi_{21}$ and $\varphi_1 \W \varphi_{22}$ can be normalized, ad we are done.

\item $\varphi_1$ has at least one \U-subformula. \\
Assume w.l.o.g. that $\varphi_2$ is in conjunctive normal form.  We proceed by induction on the number $k$ of conjuncts of 
$\varphi_2$.

\smallskip\noindent If $k=1$ then, by a similar argument to that of the previous case, we can assume that $\varphi_2 = (\psi_1 \U \psi_2 \vee \psi_3)$ for formulas $\psi_1, \psi_2,\psi_3 \in \Sigma_2$. Observe that the total number of \U-subformulas of $\psi_1, \psi_2,\psi_3$ is one less than the total number of 
$\varphi_1$ and $\varphi_2$. We have:

$$\begin{array}{cl}
&  \varphi_1 \W \varphi_2 \\
\equiv &  (\psi_1 \U \psi_2 \vee \psi_3) \W \varphi_2 \\
\equiv &  (\psi_1 \U \psi_2 \vee \psi_3) \U  (\varphi_2 \vee  \G (\psi_1 \U \psi_2 \vee \psi_3)) \\
\equiv &  (\psi_1 \U \psi_2 \vee \psi_3) \U ( \varphi_2 \vee  \G (\psi_1 \W \psi_2 \vee \psi_3) \wedge (\G\F\psi_2 \vee \G \psi_3)) \\
\equiv & (\psi_1 \U \psi_2 \vee \psi_3) \U \varphi_2  \vee  (\G(\psi_1 \W \psi_2 \vee \psi_3) \wedge  \G\F \psi_2) \vee  (\psi_1 \U \psi_2 \vee \psi_3) \U \G  \psi_3

\end{array}
$$

Since $(\psi_1 \U \psi_2 \vee \psi_3) \U \varphi_2 \in \Sigma_2$, it is already in normal form.
Since $\G (\psi_1 \W \psi_2 \vee \psi_3) = (\psi_1 \W \psi_2 \vee \psi_3) \W \false$, by induction hypothesis it can be normalized, and $\G\F\psi_2$ can be normalized by Proposition \ref{prop:boolup}. It remains to show that the third conjunct
is normalizable.  For this we first observe that $\G \psi_3 = \psi_3 \W \false$ can be normalized by induction hypothesis, and then that, after normalizing $\G\psi_3$, the formula $(\psi_1 \U \psi_2 \vee \psi_3) \U \G  \psi_3$ belongs to $Cl(\Sigma_2; \U, \G\F)$, and so can be normalized by Proposition \ref{prop:boolup}.
\end{itemize}

\end{proof}


\subsection{L(\U, \W) can be normalized}

\begin{proposition} 
Formulas of \emph{L(\U, \W)} can be normalized.
\end{proposition}
\begin{proof}
By structural induction. Since it suffices to normalize the temporal formulas, there are two cases. If $\varphi = \varphi_1 \U \varphi_2$, then $\varphi_1$ and $\varphi_2$ can be normalized by induction hypothesis, and so w.l.o.g. we can assume they are positive Boolean combinations of formulas of $\Sigma_2$ and $\G\F \Sigma_1$. Let $\varphi'$ be the result of exhaustively applying the equivalences (\ref{id1})-(\ref{id2p})to $\varphi$, as in Proposition \ref{prop:boolup}. The result is a Boolean combination of formulas of $\Sigma_2$ and formulas of $\G\F \Pi_1$, and so in normal form-.


The remaining case is $\varphi = \varphi_1 \W \varphi_2$. By induction hypothesis, $\varphi_1$ and $\varphi_2$ can be normalized, and so w.l.o.g. we can assume they are positive Boolean combinations of formulas of $\Sigma_2$ and $\G\F \Sigma_1$. Using
\begin{eqnarray}
(\psi_1 \wedge \psi_2) \W \psi_3 & \equiv & \psi_1 \W \psi_3 \wedge \psi_1 \W \psi_3 \label{id5}\\
\psi_1 \W (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \W\psi_2 \vee \psi_1 \W \psi_3 \label{id6}\\
(\psi_1 \vee \G\F \psi) \,\W \psi_2 & \equiv  & \G\F \psi \vee \psi_1 \W \psi_2  \label{id7} \\
\psi_1  \,\W (\G\F \psi \wedge \psi_2) & \equiv  &(\G\F \psi \wedge  \psi_1 \W \psi_2) \vee \G \psi_1
\end{eqnarray}

\noindent we obtain that $\varphi$ is equivalent to a positive Boolean combination of formulas in normal form and formulas 
of $\Sigma_2 \W \Sigma_2$, which can be normalized by Proposition \ref{prop:s2ws2}. 
\end{proof}

\subsection{ L(\U, \W, \X) can be normalized }

\begin{proposition} 
Formulas of \emph{L(\U, \W, \X)} can be normalized.
\end{proposition}
\begin{proof}
The identities 
$$
\begin{array}{rclcrcl}
\X(\varphi_1 \wedge \varphi_2) & \equiv & \X \varphi_1 \wedge \X \varphi_2 & \qquad   & \X(\varphi_1 \vee \varphi_2) & \equiv & \X \varphi_1 \vee  \X \varphi_2\\
\X(\varphi_1 \U \varphi_2) & \equiv & \X \varphi_1 \U \, \X \varphi_2  &  & \X(\varphi_1 \W \varphi_2) & \equiv & \X \varphi_1 \W \, \X \varphi_2
\end{array}
$$
\noindent allow us to push $\X$ across all operators. Since we can normalize all formulas of L(\U, \W), we can also normalize any formula $\varphi$ of L(\U, \W, \X) as follows:
\begin{itemize}
\item Push all occurrences of $\X$ inside $\varphi$ as much as possible.
\item Replace every maximal subformula $\X \psi$ by an atomic proposition $a_\psi$.
\item Normalize the resulting formula of L(\U,\W).
\item Replace every occurrence of $a_\psi$ in back to  $\X \psi$. The result is still in normal form, and by the Substitution Lemma it is equivalent to the original formula.
\end{itemize}
\end{proof}


Attempt:



\begin{proposition} 
\label{prop:s2ws2}
Formulas of \emph{L(\U, \W)} can be normalized.
\end{proposition}
\begin{proof}
We associate to a formula $\varphi$ a pair $\countt{\varphi} = ( \countu{\varphi}, \countw{\varphi})$, where $\countu{\varphi}$ and $\countw{\varphi}$ are the number of \U- and \W-nodes in the syntax tree of $\varphi$, respectively. We say that $\countt{\varphi} \prec \countt{\psi}$ if 
$\countu{\varphi} < \countu{\psi}$ or $\countu{\varphi} = \countu{\psi}$ and $\countw{\varphi} < \countw{\psi}$.
Clearly, $\prec$ is a well-founded partial order. We proceed by noetherian induction on $\prec$.  It suffices to consider
the cases $\varphi = \varphi_1 \U \varphi_2$ and $\varphi = \varphi_1 \W \varphi_2$, the others follow immediately from the definition of the normal form. We have $\countt{\varphi_1}  \prec \countt{\varphi}$ and $\countt{\varphi_2}  \prec \countt{\varphi}$, and so, by induction hypothesis, both $\varphi_1$ and $\varphi_2$ can be normalized. So we assume w.l.o.g. that $\varphi_1$ and $\varphi_2$ are in normal form.

If $\varphi = \varphi_1 \U \varphi_2$ then we have $\varphi_1 \U  \varphi_2 \in Cl(\Sigma_2; \U, \G\F)$, and so $\varphi$ can be normalized by Proposition \ref{prop:boolup}.  Assume now that $\varphi = \varphi_1 \W \varphi_2$.  Consider three cases.

\smallskip\noindent (a) Neither $\varphi_1$ nor $\varphi_2$ have \U-subformulas.\\
Then $\varphi_1 \W \varphi_2 \in \Pi_1$, and so in normal form.

\smallskip\noindent (b) $\varphi_2$ has at least one \U-subformula. \\
We have $\varphi_1 \W \varphi_2 \equiv   \varphi_1 \U \varphi_2 \vee  \G \varphi_1$
The formula $\varphi_1 \U  \varphi_2$ can be normalized by the argument above using Proposition \ref{prop:boolup}.  Since $\varphi_2$ has at least one \U-subformula, we have $\countt{\G \varphi_1} \prec \countt{\varphi_1 \W \varphi_2 }$. By induction hypothesis $\G \varphi_1$ can also be normalized, and we are done. 

\smallskip\noindent (c) $\varphi_2$ has no \U-subformulas, and $\varphi_1$ has at least one \U-subformula. \\
Applying exhaustively 
\begin{eqnarray}
(\psi_1 \wedge \psi_2) \W \psi_3 & \equiv & \psi_1 \W \psi_3 \wedge \psi_1 \W \psi_3 \label{id5}\\
% \psi_1 \W (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \W\psi_2 \vee \psi_1 \W \psi_3 \label{id6}\\
(\psi_1 \vee \G\F \psi) \,\W \psi_2 & \equiv  & \G\F \psi \vee \psi_1 \W \psi_2  \label{id7} 
%\psi_1  \,\W (\G\F \psi \wedge \psi_2) & \equiv  &(\G\F \psi \wedge  \psi_1 \W \psi_2) \vee \G \psi_1
\end{eqnarray}
\noindent we can transform $\varphi$ into a Boolean combination of formulas of the form
$\varphi_1 \W \varphi_2$, where $\varphi_1$ is a disjunction of atomic propositions and \U-formulas, with at least one of the latter.  So it suffices to consider this case, i.e., we can assume w.l.o.g. that $\varphi_1=(\psi_1 \U \psi_2 \vee \psi_3)$ for some $\psi_1, \psi_2,\psi_3$ in $\Sigma_2$. We have:

$$\begin{array}{cl}
&  \varphi_1 \W \varphi_2 \\
\equiv &  \varphi_1 \U  (\varphi_2 \vee  \G \varphi_1) \\
\equiv &  \varphi_1 \U  (\varphi_2 \vee  \G (\psi_1 \U \psi_2 \vee \psi_3)) \\
\equiv &  \varphi_1 \U ( \varphi_2 \vee  \G (\psi_1 \W \psi_2 \vee \psi_3) \wedge (\G\F\psi_2 \vee \G \psi_3)) \\
\equiv &  \varphi_1 \U \varphi_2  \vee  (\G(\psi_1 \W \psi_2 \vee \psi_3) \wedge  \G\F \psi_2) \vee  \varphi_1 \U \G  \psi_3
\end{array}
$$

Since $\varphi_1 \U \varphi_2 \in Cl(\Sigma_2; \U, \G\F)$, it can be normalized. Since $\G (\psi_1 \W \psi_2 \vee \psi_3) \prec  \varphi_1 \W \varphi_2$, by induction hypothesis it can also be normalized too. $\G\F\psi_2$ can be normalized by Proposition \ref{prop:boolup}. It remains to show that $\varphi_1 \U \G  \psi_3$ can be normalized.  $\G \psi_3$ can be normalized by induction hypothesis because $\G \psi_3 \prec \varphi_1 \W \varphi_2$, and so $\varphi_1 \U \G  \psi_3$ can be normalized, because it is equivalent to a formula of $Cl(\Sigma_2; \U, \G\F)$ (Proposition \ref{prop:boolup}).
\end{proof}



==> Sections/easyproof2.tex <==
\section{The Normalization Theorem}
\label{sec:overview}

\begin{definition}
\label{def:normalform}
A formula of LTL is in \emph{normal form} if it is a positive Boolean combination of formulas of 
$\Sigma_2$ and formulas of the form $\G\F \varphi$, where $\varphi \in \Sigma_1$ (and so $\G\F \varphi \in \Pi_2$). 
\end{definition}

We prove that every formula of L(\U, \W, \X) can be normalized.  A formula of 
L(\U, \W, \X) is a \emph{temporal formula} if the operator at the top of its syntax tree is
$\U$, $\W$, or $\X$.  The following fact is an imediate consequence of the definition:

\begin{factt}
\label{fact:Bool}
If all temporal formulas are normalizable, then all formulas are normalizable. 
\end{factt}

%\paragraph{Disjunctive-Conjunctive-Normalform.} Because of the identities
%$$
%\begin{array}{cc}
%(\varphi_1 \wedge \varphi_2) \Z \varphi_3 \equiv (\varphi_1 \Z \varphi_3) \wedge (\varphi_2 \Z \varphi_3) \\
%\varphi_1 \Z (\varphi_2 \vee \varphi_3 ) \equiv (\varphi_1 \Z \varphi_2) \vee (\varphi_1 \Z \varphi_3) \\
%\end{array}
%$$
%it suffices to prove the result for formulas of $L(\U, \W)$ with syntax
%$$\varphi ::=  a \mid  \left( \vee \varphi \right) \U \left( \wedge \varphi \right) \mid \left( \vee \varphi \right) \W \left( \wedge \varphi \right)$$

\subsection{$\G\F\Sigma_2$-formulas can be normalized}

The key to the normalization theorem is to observe that formulas of the form $\G\F\varphi$ satisy very special properties.

We consider formulas $\varphi$ with a ``hole'' that can be filled with a formula. 
Formally, let $\hole$ be a symbol denoting a special atomic proposition. A formula with a hole is a formula with one
single occurrence of $\hole$. We let $\varphi\hole$ denote that $\varphi$ is a formula with a hole, and denote by $\varphi[\psi]$ the result of filling the hole with $\psi$; formally, $\varphi[\psi]$ is the result of substituting $\psi$ for the unique occurrence of $\hole$ in $\varphi$. For example, if $\varphi\hole = a \W \hole$, then $\varphi[a \U c ] = a \W (a \U c)$ and $\varphi[\X b ] = a \W \X b$.

\begin{lemma}
\label{lem:GF}
For every formula $\varphi[\psi_1 \W \psi_2]$:
$$\G\F \varphi [\psi_1 \W \psi_2] \equiv (\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]) \vee  (\F\G \psi_1 \wedge \G\F \varphi [\true]) \vee \G\F \varphi [\false]$$
\end{lemma}
\begin{proof}
The proof repeatedly uses the following observation, an immediate consequence of the fact that $\varphi$ is in negation normal form:

\begin{equation}
\text{For every two formulas $\psi, \psi'$, if $\psi \models \psi'$ then  $\varphi [\psi] \models \varphi [\psi']$.} \label{sta}
\end{equation}

\noindent ($\leftmodels$)  We prove the following three claims, which immediately imply the result:
\begin{itemize}
\item $\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]  \models  \G\F \varphi [\psi_1 \W \psi_2]$. \\
Follows from $\psi_1 \U \psi_2 \models \psi_1 \W \psi_2$ and (\ref{sta}).
\item $\F\G \psi_1 \wedge \G\F \varphi [\true] \models \G\F \varphi [\psi_1 \W \psi_2]$. \\
Assume $w \models \F\G \psi_1 \wedge \G\F \varphi [\true]$. Then  infinitely many suffixes of $w$ satisfy $\G\psi_1$ and so $\varphi [\psi_1 \W \psi_2]$. These suffixes also satisfy $\psi_1 \W \psi_2$, and we are done.
\item $\G\F \varphi [\false] \models \G\F \varphi [\psi_1 \W \psi_2]$.\\
Follows from $\false \models \psi_1 \W \psi_2$ and (\ref{sta}).
\end{itemize}

\medskip

\noindent ($\models$)  Assume $w$ satisfies $\G\F \varphi [\psi_1 \W \psi_2]$, and so that  $w' \models \varphi [\psi_1 \W \psi_2]$ for infinitely many suffixes $w'$ of $w$. We prove the following three claims, which immediately imply the result:
\begin{itemize}
\item If $w \models \G\F \psi_2$ then  $w \models \G\F \varphi [\psi_1 \U \psi_2]$. \\
Since $w \models \G\F \varphi [\psi_1 \W \psi_2]$, it suffices to show that the infinitely many suffixes $w'$ of $w$ satisfying $\varphi [\psi_1 \W \psi_2]$ also satisfy $\varphi [\psi_1 \U \psi_2]$. 
For this, observe that  $w' \models \psi_1 \W \psi_2$ and  $w \models \G\F \psi_2$ imply $w' \models \psi_1 \U \psi_2$. 

\item If $w \models \F\G \psi_1$ then $w \models \G\F \varphi [\true]$.\\
Since $w \models \F\G \psi_1 \wedge \G\F \varphi [\psi_1 \W \psi_2]$, infinitely many suffixes of $w$ satisfy $\G\psi_1$ and $\varphi [\psi_1 \W \psi_2]$. Since $\G\psi_1 \models \psi_1 \W \psi_2$, these suffixes also satisfy $\psi_1 \W \psi_2$, and so also $\varphi [\true]$.

\item If $w \not\models \G\F \psi_2$ and $w \not\models \F\G \psi_1$, then $w \models \G\F \varphi [\false]$. \\
Since $w \not\models \G\F \psi_2$ and $w \not\models \F\G \psi_1$, 
infinitely many suffixes of $w$ satisfying $\varphi [\psi_1 \W \psi_2]$ do not satisfy $\psi_1 \W \psi_2$.
So they satisfy $\varphi [\false]$, which implies $w \models \G\F \varphi [\false]$.
\end{itemize}
\end{proof}

\begin{proposition}
\label{prop1}
Formulas of $\G\F \Sigma_2$ can be normalized.
\end{proposition}
\begin{proof}
Let $\G\F \varphi \in \G\F \Sigma_2$.  We prove that $\G\F \varphi$ can be normalized by induction on the number of \W-subformulas of $\varphi$. If there are none, then $\G\F\varphi \in \G\F\Pi_1$ and we are done. Otherwise, let $\psi_1 \W \psi_2$ be a  \W-subformula of $\varphi$. By Lemma \ref{lem:GF} we have
$$\G\F \varphi [\psi_1 \W \psi_2] \equiv (\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]) \vee  (\F\G \psi_1 \wedge \G\F \varphi [\true]) \vee \G\F \varphi [\false]$$
By induction hypothesis $\G\F \psi_2$, $\G\F \varphi [\psi_1 \U \psi_2]$, $\G\F\varphi [\true]$, and $\G\F \varphi [\false]$ can be normalized. Further, since $\varphi \in \Sigma_2$ we have $\psi_1 \in \Pi_1$ and $\F\G \psi_1 \in \Sigma_2$. So $\F\G \psi_1$ is also in normal form, and we are done.
\end{proof}

\subsection{L(\U, \G\F) can be normalized}

\begin{definition}
\label{prop:boolup}
$Cl(\Sigma_2; \U, \G\F)$ denotes the closure of $\Sigma_2$ under $\U$ and $\G\F$, i.e., the smallest set of formulas ${\cal F}$ satisfying: 
\begin{itemize}
\item $\Sigma_2 \subseteq {\cal F}$; 
\item if $\varphi, \psi \in {\cal F}$, then $\varphi \U \psi \in {\cal F}$; and
\item if $\varphi \in {\cal F}$, then $\G\F \varphi \in {\cal F}$.
\end{itemize}
\end{definition}

\begin{proposition}
\label{prop:boolup}
Formulas of $Cl(\Sigma_2; \U, \G\F)$ can be normalized.
\end{proposition}
\begin{proof}
Let $\varphi$ be a formula of $Cl(\Sigma_2; \U, \G\F)$. We show that $\varphi$ is equivalent to a Boolean combination
of formulas of $\Sigma_2$ and formulas of $\G\F \Sigma_2$. The result then follows from Proposition \ref{prop1}.

Let $\varphi'$ be the result of exhaustively applying the following equivalences to $\varphi$ (from left to right):

\begin{eqnarray}
(\psi_1 \wedge \psi_2) \U \psi_3 & \equiv & \psi_1 \U \psi_3 \wedge \psi_2 \U \psi_3 \label{id1}\\
\psi_1 \U (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \U \psi_2 \vee \psi_1 \U \psi_3 \label{id2}\\
(\psi_1 \vee \G\F \psi) \,\U \psi_2 & \equiv  & (\G\F \psi \wedge  \psi_2) \vee \psi_1 \U \psi_2  \label{id3}\\
\psi_1  \,\U (\G\F \psi \wedge \psi_2) & \equiv  &\G\F \psi \wedge  \psi_1 \U \varphi_2 \label{id4} \\
\G\F( \psi_1 \wedge \G\F \psi_2) &\equiv & \G\F \psi_1 \wedge \G\F \psi_2  \label{id1p}\\
\G\F( \psi_1 \vee \G\F \psi_2) &\equiv & \G\F \psi_1 \vee \G\F \psi_2  \label{id2p}\\
\G\F( \G\F\varphi) &\equiv & \G\F \varphi \label{id3p}
\end{eqnarray}

By (\ref{id1})-(\ref{id4}), no path of the syntax tree of $\varphi'$ contains a \U{} before a \G\F. By (\ref{id1p})-(\ref{id3p}),
no path of the tree contains two or more occurrences of \G\F. So the projection of every path of the syntax tree onto
\G\F, \U, and \W{} belongs to the regular expression $(\epsilon + \G\F) \U^*\W^*$. So $\varphi'$ is a Boolean combination of formulas of $\Sigma_2$ and formulas of $\G\F \Sigma_2$.

%The proof is by structural induction. By Fact \ref{fact:Bool} it
%suffices to consider two cases:
%
%\medskip
%
%\noindent Case 1: $\varphi = \G\F \varphi_1$. \\
%By induction hypothesis, $\varphi_1$ can be normalized, i.e., we can assume it is a positive Boolean combination of 
%formulas of $\Sigma_2$ and $\G\F\Sigma_1$, and w.l.o.g. that it is in disjunctive normal form. 
%We proceed by induction on the number $k$ of disjuncts of $\varphi_1$. 
%
%\medskip \noindent Base: $k=1$. Then $\varphi_1$ is a conjunction. We proceed by induction on the number of conjuncts that are formulas of $\G\F\Sigma_1$. If there are none, then $\varphi_1 \in \Sigma_2$ and the result follows from Proposition \ref{prop1}. If there is at east one, then 
%$\varphi_1 = \varphi_2 \wedge \G\F \varphi_3$ for some $\varphi_3 \in \Pi_1$. We apply
%$$\G\F \varphi_1 \equiv \G\F( \varphi_2 \wedge \G\F \varphi_3) \equiv \G\F \varphi_2 \wedge \G\F \varphi_3 \  .$$
%\noindent By induction hypothesis (induction on $\ell$), $\G\F \varphi_2$ can be normalized, and $\G\F \varphi_3$ is already in normal form, because $\varphi_3 \in \Pi_1$. So $\G\F \varphi_1$ can be normalized.
%
%\medskip \noindent Step: $k>1$. Then $\varphi_1 = \varphi_2 \vee \varphi_3$  for some formulas $\varphi_2, \varphi_3$.
%Since $\G\F (\varphi_2 \vee \varphi_3) \equiv \G\F \varphi_2 \vee \G\F \varphi_3$, by induction hypothesis (induction on $k$) the formulas $\G\F \varphi_2$ and $\G\F \varphi_3$ can be normalized, and we are done. 
%
%\bigskip\noindent Case 2: $\varphi = \varphi_1 \U \varphi_2$. By induction hypothesis, $\varphi_1$ and $\varphi_2$ can be normalized, i.e., we can assumethey are positive Boolean combinations of formulas of $\Sigma_2$ and $\G\F\Sigma_1$. By exhaustively applying the identities 
%\begin{eqnarray}
%(\psi_1 \wedge \psi_2) \U \psi_3 & \equiv & \psi_1 \U \psi_3 \wedge \psi_2 \U \psi_3 \label{id1}\\
%\psi_1 \U (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \U \psi_2 \vee \psi_1 \U \psi_3 \label{id2}\\
%(\psi_1 \vee \G\F \psi) \,\U \psi_2 & \equiv  & (\G\F \psi \wedge  \psi_2) \vee \psi_1 \U \psi_2  \label{id3}\\
%\psi_1  \,\U (\G\F \psi \wedge \psi_2) & \equiv  &\G\F \psi \wedge  \psi_1 \U \varphi_2 \label{id4}
%\end{eqnarray}
%\noindent which allow to move $\G\F$ up across $\U$, we obtain that $\varphi$ is equivalent to a positive Boolean combination of formulas of $\G\F\Sigma_1$ and formulas of the form $\psi_1 \U \psi_2$, where $\psi_1$ and $\psi_2$ have no $\G\F$-subformulas.  But then $\psi_1 \U \psi_2 \in \Sigma_1$, and we are done. 
\end{proof}

\subsection{L(\U, \W) can be normalized}

\begin{proposition}
\label{prop:s2ws2}
Formulas of \emph{L(\U, \W)} can be normalized.
\end{proposition}
\begin{proof}
We associate to a formula $\varphi$ a pair $\countt{\varphi} = ( \countu{\varphi}, \countw{\varphi})$, where $\countu{\varphi}$ and $\countw{\varphi}$ are the number of \U- and \W-nodes in the syntax tree of $\varphi$, respectively. We say that $\countt{\varphi} \prec \countt{\psi}$ if 
$\countu{\varphi} < \countu{\psi}$ or $\countu{\varphi} = \countu{\psi}$ and $\countw{\varphi} < \countw{\psi}$.
Clearly, $\prec$ is a well-founded partial order. We proceed by noetherian induction on $\prec$.  It suffices to consider
the cases $\varphi = \varphi_1 \U \varphi_2$ and $\varphi = \varphi_1 \W \varphi_2$, the others follow immediately from the definition of the normal form. We have $\countt{\varphi_1}  \prec \countt{\varphi}$ and $\countt{\varphi_2}  \prec \countt{\varphi}$, and so, by induction hypothesis, both $\varphi_1$ and $\varphi_2$ can be normalized. So we assume w.l.o.g. that $\varphi_1$ and $\varphi_2$ are in normal form.

If $\varphi = \varphi_1 \U \varphi_2$ then we have $\varphi_1 \U  \varphi_2 \in Cl(\Sigma_2; \U, \G\F)$, and so $\varphi$ can be normalized by Proposition \ref{prop:boolup}.  Assume now that $\varphi = \varphi_1 \W \varphi_2$.  Consider three cases.

\smallskip\noindent (a) Neither $\varphi_1$ nor $\varphi_2$ have \U-subformulas.\\
Then $\varphi_1 \W \varphi_2 \in \Pi_1$, and so in normal form.

\smallskip\noindent (b) $\varphi_2$ has at least one \U-subformula. \\
We have $\varphi_1 \W \varphi_2 \equiv   \varphi_1 \U \varphi_2 \vee  \G \varphi_1$
The formula $\varphi_1 \U  \varphi_2$ can be normalized by the argument above using Proposition \ref{prop:boolup}.  Since $\varphi_2$ has at least one \U-subformula, we have $\countt{\G \varphi_1} \prec \countt{\varphi_1 \W \varphi_2 }$. By induction hypothesis $\G \varphi_1$ can also be normalized, and we are done. 

\smallskip\noindent (c) $\varphi_2$ has no \U-subformulas, and $\varphi_1$ has at least one \U-subformula. \\
Applying exhaustively 
\begin{eqnarray}
(\psi_1 \wedge \psi_2) \W \psi_3 & \equiv & \psi_1 \W \psi_3 \wedge \psi_1 \W \psi_3 \label{id5}\\
% \psi_1 \W (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \W\psi_2 \vee \psi_1 \W \psi_3 \label{id6}\\
(\psi_1 \vee \G\F \psi) \,\W \psi_2 & \equiv  & \G\F \psi \vee \psi_1 \W \psi_2  \label{id7} 
%\psi_1  \,\W (\G\F \psi \wedge \psi_2) & \equiv  &(\G\F \psi \wedge  \psi_1 \W \psi_2) \vee \G \psi_1
\end{eqnarray}
\noindent we can transform $\varphi$ into a Boolean combination of formulas of the form
$\varphi_1 \W \varphi_2$, where $\varphi_1$ is a disjunction of atomic propositions and \U-formulas, with at least one of the latter.  So it suffices to consider this case, i.e., we can assume w.l.o.g. that $\varphi_1=(\psi_1 \U \psi_2 \vee \psi_3)$ for some $\psi_1, \psi_2,\psi_3$ in $\Sigma_2$. We have:

$$\begin{array}{cl}
&  \varphi_1 \W \varphi_2 \\
\equiv &  \varphi_1 \U  (\varphi_2 \vee  \G \varphi_1) \\
\equiv &  \varphi_1 \U  (\varphi_2 \vee  \G (\psi_1 \U \psi_2 \vee \psi_3)) \\
\equiv &  \varphi_1 \U ( \varphi_2 \vee  \G (\psi_1 \W \psi_2 \vee \psi_3) \wedge (\G\F\psi_2 \vee \G \psi_3)) \\
\equiv &  \varphi_1 \U \varphi_2  \vee  (\G(\psi_1 \W \psi_2 \vee \psi_3) \wedge  \G\F \psi_2) \vee  \varphi_1 \U \G  \psi_3
\end{array}
$$

Since $\varphi_1 \U \varphi_2 \in Cl(\Sigma_2; \U, \G\F)$, it can be normalized. Since $\G (\psi_1 \W \psi_2 \vee \psi_3) \prec  \varphi_1 \W \varphi_2$, by induction hypothesis it can also be normalized too. $\G\F\psi_2$ can be normalized by Proposition \ref{prop:boolup}. It remains to show that $\varphi_1 \U \G  \psi_3$ can be normalized.  $\G \psi_3$ can be normalized by induction hypothesis because $\G \psi_3 \prec \varphi_1 \W \varphi_2$, and so $\varphi_1 \U \G  \psi_3$ can be normalized, because it is equivalent to a formula of $Cl(\Sigma_2; \U, \G\F)$ (Proposition \ref{prop:boolup}).
\end{proof}


\subsection{ L(\U, \W, \X) can be normalized }

\begin{proposition} 
Formulas of \emph{L(\U, \W, \X)} can be normalized.
\end{proposition}
\begin{proof}
The identities 
$$
\begin{array}{rclcrcl}
\X(\varphi_1 \wedge \varphi_2) & \equiv & \X \varphi_1 \wedge \X \varphi_2 & \qquad   & \X(\varphi_1 \vee \varphi_2) & \equiv & \X \varphi_1 \vee  \X \varphi_2\\
\X(\varphi_1 \U \varphi_2) & \equiv & \X \varphi_1 \U \, \X \varphi_2  &  & \X(\varphi_1 \W \varphi_2) & \equiv & \X \varphi_1 \W \, \X \varphi_2
\end{array}
$$
\noindent allow us to push $\X$ across all operators. Since we can normalize all formulas of L(\U, \W), we can also normalize any formula $\varphi$ of L(\U, \W, \X) as follows:
\begin{itemize}
\item Push all occurrences of $\X$ inside $\varphi$ as much as possible.
\item Replace every maximal subformula $\X \psi$ by an atomic proposition $a_\psi$.
\item Normalize the resulting formula of L(\U,\W).
\item Replace every occurrence of $a_\psi$ in back to  $\X \psi$. The result is still in normal form, and by the Substitution Lemma it is equivalent to the original formula.
\end{itemize}
\end{proof}





==> Sections/easyproof3.tex <==
\section{The Normalization Theorem}
\label{sec:overview}
\newcommand{\nnodes}[1]{\#({#1})}
\newcommand{\gfba}[1]{\#_{\G\F}({#1})}
\newcommand{\ubw}[1]{\#_{\U}({#1})}
\newcommand{\wbgf}[1]{\#_{\W}({#1})}

Let $\varphi$ be a formula. The syntax tree $T_\varphi$ of $\varphi$ is defined in the usual way.  We say 
that a node of $T_\varphi$ is a \emph{\U-node} if the subformula rooted at it is  a \U-formula; \W-nodes and \GF-nodes are defined similarly. We introduce four parameters:
\begin{itemize}
\item $\nnodes{\varphi}$: number of nodes of $T_\varphi$, not counting leaves labeled with $\true$ or $\false$. 
\item$\gfba{\varphi}$: number of \G\F-nodes of $T_\varphi$ that are proper descendants of some \U, \W, or \G\F-node.
\item $\wbgf{\varphi}$: number of  \W-nodes of $T_\varphi$ that are proper descendants of some \G\F-node.
\item $\ubw{\varphi}$: number of \U-nodes of $T_\varphi$ that are descendants of some \W-node.
\end{itemize}

\begin{definition}
The \emph{rank} of a formula is defined as follows:
	\[ \mathit{rank}(\varphi) = \nnodes{\varphi} + \gfba{\varphi} + \wbgf{\varphi} + \ubw{\varphi}  \]
\end{definition}

Observe that a formula is in normal form if{}f  $\mathit{rank}(\varphi) = \nnodes{\varphi}$.
We prove that every formula is normalizable by induction on the rank.

\begin{theorem}
Every formula of LTL is normalizable. 
\end{theorem}
\begin{proof}
By induction on the rank. We consider several cases.

\medskip\noindent If $\varphi = \true$ or $\varphi=\false$ then $\varphi$ is already in normal form.

\medskip\noindent If $\varphi = \varphi_1 \wedge \varphi_2$ or $\varphi = \varphi_1 \vee \varphi_2$, then by induction hypothesis
	$\varphi_1$ and $\varphi_2$  can be normalized into formulas $\varphi_1'$ and $\varphi_2'$, and so $\varphi$ can be normalized into $\varphi_1'  \wedge \varphi_2'$ or $\varphi_1' \vee \varphi_2'$, respectively.

\medskip\noindent If $\varphi  = \X \varphi_1$, then by induction hypothesis
	$\varphi_1$ can be normalized into $\varphi_1'$, and so $\varphi$ can be normalized into $\X \varphi_1'$. \todo{R: According to \cref{def:normalform}, we also have to extract $\GF$ from $\X$.}
	
\medskip\noindent  If $\varphi = \GF \varphi_1$, we consider several cases. If $\varphi_1$ contains neither \GF-nodes nor \W-nodes, 
then $\varphi$ is already in normal form. If $\varphi_1$ contains a \GF-node, say $\G\F\psi$, then by \cref{lemma:GF1} we have 
$$\GF \varphi_1[\G\F \psi] \equiv (\GF \psi \wedge \GF \varphi_1[\true]) \vee \GF \varphi_1[\false]$$
\noindent and 
since $\GF \psi$, $\GF \varphi_1[\true]$, and $\GF \varphi_1[\false]$ all contain fewer nodes than $\varphi$, they can be normalized, and we are done. If $\varphi_1$ contains a \W-node, then let $\psi_1 \W \psi_2$ be a maximal 
subformula of $\varphi_1$ (with respect to the subformula order). If $\psi_2 = \true$ then 
$\GF \varphi_1[\psi_1 \W \psi_2] \equiv \GF \varphi[\true]$, which has fewer nodes. Otherwise, 
applying \cref{lemma:GF2} we get
%
\[ \GF \varphi_1[\psi_1 \W \psi_2] \equiv (\GF \psi_2 \wedge \GF \varphi_1[\psi_1 \U \psi_2]) \vee (\F \G \psi_1 \wedge \GF \varphi_1[\true]) \vee \GF \varphi_1[\false] \]
%
$\GF \psi_2$ has fewer nodes than $\varphi$,  $\GF \varphi[\psi_1 \U \psi_2]$ has fewer \W-nodes  under \GF-nodes, and  all of  $\F \G \psi_1$, $\GF \varphi[\true]$ and $\GF \varphi[\false]$ have fewer nodes. Hence, all these subformulas can be normalized by induction hypothesis, and we are done.

\medskip\noindent If $\varphi = \varphi_1 \U \varphi_2$, then by induction hypothesis $\varphi_1$ and $\varphi_2$ can be normalized into $\varphi_1'$ and $\varphi_2'$. We show that $\varphi_1' \U \varphi_2'$ can be normalized by induction on the total number of \G\F-nodes in $\varphi_1'$ and $\varphi_2'$. If the number is $0$, then we have $\varphi_1', \varphi_2' \in \Sigma_2$; hence $\varphi_1' \U \varphi_2' \in \Sigma_2$, and so it is already in normal form. If $\varphi_1'$ has a \G\F-subformula, say $\G\F\psi$, then  by \cref{lemma:GF1}(\ref{eqGF1}) we have 
$$\varphi_1'[\G\F \psi] \U \varphi_2' \equiv (\GF \psi \wedge \varphi_1'[\true] \U \varphi_2') \vee \varphi_1'[\false] \U \varphi_2'  \ . $$ 
\noindent Since $\GF \psi$ is already in normal form (because $\varphi_1'[\G\F \psi]$ is in normal form), and $\varphi_1'[\true]$ and $\varphi_1'[\false]$ have fewer \G\F-nodes than $\varphi_1'[\G\F \psi]$, the formula $\varphi_1' \U \varphi_2'$ can be normalized. The same can be applied to $\varphi_2'$.

\medskip\noindent If $\varphi = \varphi_1 \W \varphi_2$, but $\varphi$ is not a \GF-formula, we consider several cases.
\begin{itemize}

\item Neither $\varphi_1$ nor $\varphi_2$ contain $\U$-nodes. Then $\varphi_1 \W \varphi_2$ is already in normal form. \todo[inline]{R: $\varphi_1$ and $\varphi_2$ may still contain $\GF$ nodes. Maybe we can say that $\GF$ nodes are removed like in the $\U$ case.}

\item $\varphi_2$ contains at least one $\U$-node. \todo{R: not inside a $\GF$ node?} Then $\varphi_2$ contains a maximal subformula $\psi_1 \U \psi_2$ (with respect to the subformula order). By \cref{lem:UWandWU}(\ref{eqWU}) we have 
%
	\[ \varphi_1 \W \varphi_2[\psi_1 \U \psi_2] \equiv \varphi_1 \U \varphi_2[\psi_1 \U \psi_2] \wedge \G \varphi_2[\psi_1 \U \psi_2] \]
%
By the maximality of $\psi_1 \U \psi_2$, the first conjunct has fewer $\U$-nodes under $\W$-nodes, so it can be normalized by induction hypothesis. \todo[inline]{R: the maximality is not enough to ensure that the number decreases ($a \W (b \W (c \U d))$). Maybe we should fix only all $\U$ that are not inside another $\W$.} For the second conjunct, consider three cases: if $\varphi_1 = \true$ then $\varphi \equiv \true$, which is in normal form; if $\varphi_1 = \false$, then $\varphi \equiv \varphi_2$, which can be normalized by induction hypothesis (one \W-node less); otherwise, the second conjunct has fewer nodes than $\varphi$, because $\varphi_1$ has been removed, and so it can be normalized by induction hypothesis.

\item $\varphi_1$ contains at least one \U-node. Then $\varphi_1$ contains a maximal subformula $\psi_1 \U \psi_2$ (with respect to the subformula order).  By \cref{lem:UWandWU}(\ref{eqUW})  we have
%
	\[ \begin{array}{lll}
		\varphi_1[\psi_1 \U \psi_2] \W \varphi_2 \equiv
		&  & \varphi_1[\psi_1 \U \psi_2] \U \varphi_2  \\[1ex]
		& \vee & (\GF \psi_2 \wedge \G \varphi_1[\psi_1 \W \psi_2]) \\[1ex]
		& \vee & \varphi_1[\psi_1 \U \psi_2] \, \U \, \G \varphi_1[\false]
	\end{array} \]
%
The first disjunct has fewer \U-nodes under \W-nodes than $\varphi$, \todo{R: the same problem with maximality not being enough.} and so it can be normalized by induction hypothesis. For the second disjunct, observe that
$\GF \psi_2$ has fewer nodes than $\varphi$, because otherwise we would have $\varphi_1 \W \varphi_2 = \G\F \psi_2$, contradicting the hypothesis that $\varphi$ is not a \GF-formula; further, $\G \varphi_1[\psi_1 \W \psi_2]$ has fewer \U-nodes under \W-nodes; so both can be normalized, and we are done. For the third conjunct, both $\varphi[\psi_1 \U \psi_2]$ and $\G \varphi_1[\false]$ have fewer nodes than $\varphi$, so both can be normalized, and we proceed as in the case $\varphi = \varphi_1 \U \varphi_2$ to complete the normalization.
\end{itemize}



************ Removed by Javier, check ***************

It remains to consider $\F \G \psi_1$, which has fewer operator than the original term unless $\psi_2$ is a constant. 

JAVIER: No (I think) , $\GF \varphi[\psi_1 \W \psi_2]$ has three nodes plus the nodes of $\psi_1$ and $\psi_2$,
 and $\F \G \psi_1$ has only two nodes plus the nodes of $\psi_1$.
 
RUBÉN: I counted $\GF$ as one, but I have not found any problem in the rest of the proof counting it as two. Perhaps we should say it explicitly.
 
If $\varphi_2 = \true$, the whole $\W$ operator is equivalent to $\true$ and can be trivially removed. If $\varphi_2 = \false$, the operator is a $\G$ and we have to compare $\GF \varphi[\G \psi_1]$ and $\F \G \psi_1$. However, they would only have the same number of operators if the first is $\GF \G \psi_1 \equiv \F \G \psi_1$, which we would have treated as another case.

\end{proof}


%We prove that every formula of L(\U, \W, \X) can be normalized.  A formula of 
%L(\U, \W, \X) is a \emph{temporal formula} if the operator at the top of its syntax tree is
%$\U$, $\W$, or $\X$.  The following fact is an imediate consequence of the definition:
%
%\begin{factt}
%\label{fact:Bool}
%If all temporal formulas are normalizable, then all formulas are normalizable. 
%\end{factt}
%
%%\paragraph{Disjunctive-Conjunctive-Normalform.} Because of the identities
%%$$
%%\begin{array}{cc}
%%(\varphi_1 \wedge \varphi_2) \Z \varphi_3 \equiv (\varphi_1 \Z \varphi_3) \wedge (\varphi_2 \Z \varphi_3) \\
%%\varphi_1 \Z (\varphi_2 \vee \varphi_3 ) \equiv (\varphi_1 \Z \varphi_2) \vee (\varphi_1 \Z \varphi_3) \\
%%\end{array}
%%$$
%%it suffices to prove the result for formulas of $L(\U, \W)$ with syntax
%%$$\varphi ::=  a \mid  \left( \vee \varphi \right) \U \left( \wedge \varphi \right) \mid \left( \vee \varphi \right) \W \left( \wedge \varphi \right)$$
%
%\subsection{$\G\F\Sigma_2$-formulas can be normalized}
%
%The key to the normalization theorem is to observe that formulas of the form $\G\F\varphi$ satisy very special properties.
%
%We consider formulas $\varphi$ with a ``hole'' that can be filled with a formula. 
%Formally, let $\hole$ be a symbol denoting a special atomic proposition. A formula with a hole is a formula with one
%single occurrence of $\hole$. We let $\varphi\hole$ denote that $\varphi$ is a formula with a hole, and denote by $\varphi[\psi]$ the result of filling the hole with $\psi$; formally, $\varphi[\psi]$ is the result of substituting $\psi$ for the unique occurrence of $\hole$ in $\varphi$. For example, if $\varphi\hole = a \W \hole$, then $\varphi[a \U c ] = a \W (a \U c)$ and $\varphi[\X b ] = a \W \X b$.
%
%\begin{lemma}
%\label{lem:GF}
%For every formula $\varphi[\psi_1 \W \psi_2]$:
%$$\G\F \varphi [\psi_1 \W \psi_2] \equiv (\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]) \vee  (\F\G \psi_1 \wedge \G\F \varphi [\true]) \vee \G\F \varphi [\false]$$
%\end{lemma}
%\begin{proof}
%The proof repeatedly uses the following observation, an immediate consequence of the fact that $\varphi$ is in negation normal form:
%
%\begin{equation}
%\text{For every two formulas $\psi, \psi'$, if $\psi \models \psi'$ then  $\varphi [\psi] \models \varphi [\psi']$.} \label{sta}
%\end{equation}
%
%\noindent ($\leftmodels$)  We prove the following three claims, which immediately imply the result:
%\begin{itemize}
%\item $\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]  \models  \G\F \varphi [\psi_1 \W \psi_2]$. \\
%Follows from $\psi_1 \U \psi_2 \models \psi_1 \W \psi_2$ and (\ref{sta}).
%\item $\F\G \psi_1 \wedge \G\F \varphi [\true] \models \G\F \varphi [\psi_1 \W \psi_2]$. \\
%Assume $w \models \F\G \psi_1 \wedge \G\F \varphi [\true]$. Then  infinitely many suffixes of $w$ satisfy $\G\psi_1$ and so $\varphi [\psi_1 \W \psi_2]$. These suffixes also satisfy $\psi_1 \W \psi_2$, and we are done.
%\item $\G\F \varphi [\false] \models \G\F \varphi [\psi_1 \W \psi_2]$.\\
%Follows from $\false \models \psi_1 \W \psi_2$ and (\ref{sta}).
%\end{itemize}
%
%\medskip
%
%\noindent ($\models$)  Assume $w$ satisfies $\G\F \varphi [\psi_1 \W \psi_2]$, and so that  $w' \models \varphi [\psi_1 \W \psi_2]$ for infinitely many suffixes $w'$ of $w$. We prove the following three claims, which immediately imply the result:
%\begin{itemize}
%\item If $w \models \G\F \psi_2$ then  $w \models \G\F \varphi [\psi_1 \U \psi_2]$. \\
%Since $w \models \G\F \varphi [\psi_1 \W \psi_2]$, it suffices to show that the infinitely many suffixes $w'$ of $w$ satisfying $\varphi [\psi_1 \W \psi_2]$ also satisfy $\varphi [\psi_1 \U \psi_2]$. 
%For this, observe that  $w' \models \psi_1 \W \psi_2$ and  $w \models \G\F \psi_2$ imply $w' \models \psi_1 \U \psi_2$. 
%
%\item If $w \models \F\G \psi_1$ then $w \models \G\F \varphi [\true]$.\\
%Since $w \models \F\G \psi_1 \wedge \G\F \varphi [\psi_1 \W \psi_2]$, infinitely many suffixes of $w$ satisfy $\G\psi_1$ and $\varphi [\psi_1 \W \psi_2]$. Since $\G\psi_1 \models \psi_1 \W \psi_2$, these suffixes also satisfy $\psi_1 \W \psi_2$, and so also $\varphi [\true]$.
%
%\item If $w \not\models \G\F \psi_2$ and $w \not\models \F\G \psi_1$, then $w \models \G\F \varphi [\false]$. \\
%Since $w \not\models \G\F \psi_2$ and $w \not\models \F\G \psi_1$, 
%infinitely many suffixes of $w$ satisfying $\varphi [\psi_1 \W \psi_2]$ do not satisfy $\psi_1 \W \psi_2$.
%So they satisfy $\varphi [\false]$, which implies $w \models \G\F \varphi [\false]$.
%\end{itemize}
%\end{proof}
%
%\begin{proposition}
%\label{prop1}
%Formulas of $\G\F \Sigma_2$ can be normalized.
%\end{proposition}
%\begin{proof}
%Let $\G\F \varphi \in \G\F \Sigma_2$.  We prove that $\G\F \varphi$ can be normalized by induction on the number of \W-subformulas of $\varphi$. If there are none, then $\G\F\varphi \in \G\F\Pi_1$ and we are done. Otherwise, let $\psi_1 \W \psi_2$ be a  \W-subformula of $\varphi$. By Lemma \ref{lem:GF} we have
%$$\G\F \varphi [\psi_1 \W \psi_2] \equiv (\G\F \psi_2 \wedge \G\F \varphi [\psi_1 \U \psi_2]) \vee  (\F\G \psi_1 \wedge \G\F \varphi [\true]) \vee \G\F \varphi [\false]$$
%By induction hypothesis $\G\F \psi_2$, $\G\F \varphi [\psi_1 \U \psi_2]$, $\G\F\varphi [\true]$, and $\G\F \varphi [\false]$ can be normalized. Further, since $\varphi \in \Sigma_2$ we have $\psi_1 \in \Pi_1$ and $\F\G \psi_1 \in \Sigma_2$. So $\F\G \psi_1$ is also in normal form, and we are done.
%\end{proof}
%
%\subsection{L(\U, \G\F) can be normalized}
%
%\begin{definition}
%\label{prop:boolup}
%$Cl(\Sigma_2; \U, \G\F)$ denotes the closure of $\Sigma_2$ under $\U$ and $\G\F$, i.e., the smallest set of formulas ${\cal F}$ satisfying: 
%\begin{itemize}
%\item $\Sigma_2 \subseteq {\cal F}$; 
%\item if $\varphi, \psi \in {\cal F}$, then $\varphi \U \psi \in {\cal F}$; and
%\item if $\varphi \in {\cal F}$, then $\G\F \varphi \in {\cal F}$.
%\end{itemize}
%\end{definition}
%
%\begin{proposition}
%\label{prop:boolup}
%Formulas of $Cl(\Sigma_2; \U, \G\F)$ can be normalized.
%\end{proposition}
%\begin{proof}
%Let $\varphi$ be a formula of $Cl(\Sigma_2; \U, \G\F)$. We show that $\varphi$ is equivalent to a Boolean combination
%of formulas of $\Sigma_2$ and formulas of $\G\F \Sigma_2$. The result then follows from Proposition \ref{prop1}.
%
%Let $\varphi'$ be the result of exhaustively applying the following equivalences to $\varphi$ (from left to right):
%
%\begin{eqnarray}
%(\psi_1 \wedge \psi_2) \U \psi_3 & \equiv & \psi_1 \U \psi_3 \wedge \psi_2 \U \psi_3 \label{id1}\\
%\psi_1 \U (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \U \psi_2 \vee \psi_1 \U \psi_3 \label{id2}\\
%(\psi_1 \vee \G\F \psi) \,\U \psi_2 & \equiv  & (\G\F \psi \wedge  \psi_2) \vee \psi_1 \U \psi_2  \label{id3}\\
%\psi_1  \,\U (\G\F \psi \wedge \psi_2) & \equiv  &\G\F \psi \wedge  \psi_1 \U \varphi_2 \label{id4} \\
%\G\F( \psi_1 \wedge \G\F \psi_2) &\equiv & \G\F \psi_1 \wedge \G\F \psi_2  \label{id1p}\\
%\G\F( \psi_1 \vee \G\F \psi_2) &\equiv & \G\F \psi_1 \vee \G\F \psi_2  \label{id2p}\\
%\G\F( \G\F\varphi) &\equiv & \G\F \varphi \label{id3p}
%\end{eqnarray}
%
%By (\ref{id1})-(\ref{id4}), no path of the syntax tree of $\varphi'$ contains a \U{} before a \G\F. By (\ref{id1p})-(\ref{id3p}),
%no path of the tree contains two or more occurrences of \G\F. So the projection of every path of the syntax tree onto
%\G\F, \U, and \W{} belongs to the regular expression $(\epsilon + \G\F) \U^*\W^*$. So $\varphi'$ is a Boolean combination of formulas of $\Sigma_2$ and formulas of $\G\F \Sigma_2$.
%
%%The proof is by structural induction. By Fact \ref{fact:Bool} it
%%suffices to consider two cases:
%%
%%\medskip
%%
%%\noindent Case 1: $\varphi = \G\F \varphi_1$. \\
%%By induction hypothesis, $\varphi_1$ can be normalized, i.e., we can assume it is a positive Boolean combination of 
%%formulas of $\Sigma_2$ and $\G\F\Sigma_1$, and w.l.o.g. that it is in disjunctive normal form. 
%%We proceed by induction on the number $k$ of disjuncts of $\varphi_1$. 
%%
%%\medskip \noindent Base: $k=1$. Then $\varphi_1$ is a conjunction. We proceed by induction on the number of conjuncts that are formulas of $\G\F\Sigma_1$. If there are none, then $\varphi_1 \in \Sigma_2$ and the result follows from Proposition \ref{prop1}. If there is at east one, then 
%%$\varphi_1 = \varphi_2 \wedge \G\F \varphi_3$ for some $\varphi_3 \in \Pi_1$. We apply
%%$$\G\F \varphi_1 \equiv \G\F( \varphi_2 \wedge \G\F \varphi_3) \equiv \G\F \varphi_2 \wedge \G\F \varphi_3 \  .$$
%%\noindent By induction hypothesis (induction on $\ell$), $\G\F \varphi_2$ can be normalized, and $\G\F \varphi_3$ is already in normal form, because $\varphi_3 \in \Pi_1$. So $\G\F \varphi_1$ can be normalized.
%%
%%\medskip \noindent Step: $k>1$. Then $\varphi_1 = \varphi_2 \vee \varphi_3$  for some formulas $\varphi_2, \varphi_3$.
%%Since $\G\F (\varphi_2 \vee \varphi_3) \equiv \G\F \varphi_2 \vee \G\F \varphi_3$, by induction hypothesis (induction on $k$) the formulas $\G\F \varphi_2$ and $\G\F \varphi_3$ can be normalized, and we are done. 
%%
%%\bigskip\noindent Case 2: $\varphi = \varphi_1 \U \varphi_2$. By induction hypothesis, $\varphi_1$ and $\varphi_2$ can be normalized, i.e., we can assumethey are positive Boolean combinations of formulas of $\Sigma_2$ and $\G\F\Sigma_1$. By exhaustively applying the identities 
%%\begin{eqnarray}
%%(\psi_1 \wedge \psi_2) \U \psi_3 & \equiv & \psi_1 \U \psi_3 \wedge \psi_2 \U \psi_3 \label{id1}\\
%%\psi_1 \U (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \U \psi_2 \vee \psi_1 \U \psi_3 \label{id2}\\
%%(\psi_1 \vee \G\F \psi) \,\U \psi_2 & \equiv  & (\G\F \psi \wedge  \psi_2) \vee \psi_1 \U \psi_2  \label{id3}\\
%%\psi_1  \,\U (\G\F \psi \wedge \psi_2) & \equiv  &\G\F \psi \wedge  \psi_1 \U \varphi_2 \label{id4}
%%\end{eqnarray}
%%\noindent which allow to move $\G\F$ up across $\U$, we obtain that $\varphi$ is equivalent to a positive Boolean combination of formulas of $\G\F\Sigma_1$ and formulas of the form $\psi_1 \U \psi_2$, where $\psi_1$ and $\psi_2$ have no $\G\F$-subformulas.  But then $\psi_1 \U \psi_2 \in \Sigma_1$, and we are done. 
%\end{proof}
%
%\subsection{L(\U, \W) can be normalized}
%
%\begin{proposition}
%\label{prop:s2ws2}
%Formulas of \emph{L(\U, \W)} can be normalized.
%\end{proposition}
%\begin{proof}
%We associate to a formula $\varphi$ a pair $\countt{\varphi} = ( \countu{\varphi}, \countw{\varphi})$, where $\countu{\varphi}$ and $\countw{\varphi}$ are the number of \U- and \W-nodes in the syntax tree of $\varphi$, respectively. We say that $\countt{\varphi} \prec \countt{\psi}$ if 
%$\countu{\varphi} < \countu{\psi}$ or $\countu{\varphi} = \countu{\psi}$ and $\countw{\varphi} < \countw{\psi}$.
%Clearly, $\prec$ is a well-founded partial order. We proceed by noetherian induction on $\prec$.  It suffices to consider
%the cases $\varphi = \varphi_1 \U \varphi_2$ and $\varphi = \varphi_1 \W \varphi_2$, the others follow immediately from the definition of the normal form. We have $\countt{\varphi_1}  \prec \countt{\varphi}$ and $\countt{\varphi_2}  \prec \countt{\varphi}$, and so, by induction hypothesis, both $\varphi_1$ and $\varphi_2$ can be normalized. So we assume w.l.o.g. that $\varphi_1$ and $\varphi_2$ are in normal form.
%
%If $\varphi = \varphi_1 \U \varphi_2$ then we have $\varphi_1 \U  \varphi_2 \in Cl(\Sigma_2; \U, \G\F)$, and so $\varphi$ can be normalized by Proposition \ref{prop:boolup}.  Assume now that $\varphi = \varphi_1 \W \varphi_2$.  Consider three cases.
%
%\smallskip\noindent (a) Neither $\varphi_1$ nor $\varphi_2$ have \U-subformulas.\\
%Then $\varphi_1 \W \varphi_2 \in \Pi_1$, and so in normal form.
%
%\smallskip\noindent (b) $\varphi_2$ has at least one \U-subformula. \\
%We have $\varphi_1 \W \varphi_2 \equiv   \varphi_1 \U \varphi_2 \vee  \G \varphi_1$
%The formula $\varphi_1 \U  \varphi_2$ can be normalized by the argument above using Proposition \ref{prop:boolup}.  Since $\varphi_2$ has at least one \U-subformula, we have $\countt{\G \varphi_1} \prec \countt{\varphi_1 \W \varphi_2 }$. By induction hypothesis $\G \varphi_1$ can also be normalized, and we are done. 
%
%\smallskip\noindent (c) $\varphi_2$ has no \U-subformulas, and $\varphi_1$ has at least one \U-subformula. \\
%Applying exhaustively 
%\begin{eqnarray}
%(\psi_1 \wedge \psi_2) \W \psi_3 & \equiv & \psi_1 \W \psi_3 \wedge \psi_1 \W \psi_3 \label{id5}\\
%% \psi_1 \W (\psi_2 \vee \psi_3 ) & \equiv & \psi_1 \W\psi_2 \vee \psi_1 \W \psi_3 \label{id6}\\
%(\psi_1 \vee \G\F \psi) \,\W \psi_2 & \equiv  & \G\F \psi \vee \psi_1 \W \psi_2  \label{id7} 
%%\psi_1  \,\W (\G\F \psi \wedge \psi_2) & \equiv  &(\G\F \psi \wedge  \psi_1 \W \psi_2) \vee \G \psi_1
%\end{eqnarray}
%\noindent we can transform $\varphi$ into a Boolean combination of formulas of the form
%$\varphi_1 \W \varphi_2$, where $\varphi_1$ is a disjunction of atomic propositions and \U-formulas, with at least one of the latter.  So it suffices to consider this case, i.e., we can assume w.l.o.g. that $\varphi_1=(\psi_1 \U \psi_2 \vee \psi_3)$ for some $\psi_1, \psi_2,\psi_3$ in $\Sigma_2$. We have:
%
%$$\begin{array}{cl}
%&  \varphi_1 \W \varphi_2 \\
%\equiv &  \varphi_1 \U  (\varphi_2 \vee  \G \varphi_1) \\
%\equiv &  \varphi_1 \U  (\varphi_2 \vee  \G (\psi_1 \U \psi_2 \vee \psi_3)) \\
%\equiv &  \varphi_1 \U ( \varphi_2 \vee  \G (\psi_1 \W \psi_2 \vee \psi_3) \wedge (\G\F\psi_2 \vee \G \psi_3)) \\
%\equiv &  \varphi_1 \U \varphi_2  \vee  (\G(\psi_1 \W \psi_2 \vee \psi_3) \wedge  \G\F \psi_2) \vee  \varphi_1 \U \G  \psi_3
%\end{array}
%$$
%
%Since $\varphi_1 \U \varphi_2 \in Cl(\Sigma_2; \U, \G\F)$, it can be normalized. Since $\G (\psi_1 \W \psi_2 \vee \psi_3) \prec  \varphi_1 \W \varphi_2$, by induction hypothesis it can also be normalized too. $\G\F\psi_2$ can be normalized by Proposition \ref{prop:boolup}. It remains to show that $\varphi_1 \U \G  \psi_3$ can be normalized.  $\G \psi_3$ can be normalized by induction hypothesis because $\G \psi_3 \prec \varphi_1 \W \varphi_2$, and so $\varphi_1 \U \G  \psi_3$ can be normalized, because it is equivalent to a formula of $Cl(\Sigma_2; \U, \G\F)$ (Proposition \ref{prop:boolup}).
%\end{proof}
%
%
%\subsection{ L(\U, \W, \X) can be normalized }
%
%\begin{proposition} 
%Formulas of \emph{L(\U, \W, \X)} can be normalized.
%\end{proposition}
%\begin{proof}
%The identities 
%$$
%\begin{array}{rclcrcl}
%\X(\varphi_1 \wedge \varphi_2) & \equiv & \X \varphi_1 \wedge \X \varphi_2 & \qquad   & \X(\varphi_1 \vee \varphi_2) & \equiv & \X \varphi_1 \vee  \X \varphi_2\\
%\X(\varphi_1 \U \varphi_2) & \equiv & \X \varphi_1 \U \, \X \varphi_2  &  & \X(\varphi_1 \W \varphi_2) & \equiv & \X \varphi_1 \W \, \X \varphi_2
%\end{array}
%$$
%\noindent allow us to push $\X$ across all operators. Since we can normalize all formulas of L(\U, \W), we can also normalize any formula $\varphi$ of L(\U, \W, \X) as follows:
%\begin{itemize}
%\item Push all occurrences of $\X$ inside $\varphi$ as much as possible.
%\item Replace every maximal subformula $\X \psi$ by an atomic proposition $a_\psi$.
%\item Normalize the resulting formula of L(\U,\W).
%\item Replace every occurrence of $a_\psi$ in back to  $\X \psi$. The result is still in normal form, and by the Substitution Lemma it is equivalent to the original formula.
%\end{itemize}
%\end{proof}
%
%
%


==> Sections/motivation.tex <==


We consider the protocol of \cite{} for the predicate $x - y \geq 2^k$. The states are triples of the form 
$(\ell, b, u)$, where $\ell, b \in \{0,1\}$ and $-2^k \leq u \leq 2^k$. Intuitively, $\ell$ indicates if 
the agent is active or passive, $b$ indicates if the agent currently believes that the predicate holds or not, and
$u$ indicates the agent's wealth, which can also be negative. Initially, all agents are active and their beliefs are negative. The accounts of agents  for the input $x$ resp. $y$ have balance $1$ resp. $-1$. So the predicate holds if{}f the total wealth of the agents is at least $2^k$.

If two passive agents meet, then their encounter has no effect. If at least one agent is active, then the result of the encounter 
is given by the transition
$$(\ell, b, u), (\ell', b', u') \mapsto (1, b'', q), (0, b, r)$$
where $b'' = 1$ if{}f $u+u' \geq 2^k$ else $0$; $q= \max(-2^k, \min(2^k, u+u'))$; and $r = u+u' - q$. 
Intuitively, after the encounter exacty one agent remains active. Further, the agents compare their joint wealth $u+u'$, with $2^k$, and update their beliefs accordingly. Finally, the active agent takes as much of $u+u'$ as possible, and the passive  agent keeps the rest. In particular, the total wealth of the agents does not change.

Correctness is proved in three steps. First, it is eay to see that eventually one singe agent remains active. Further, the wealth of this agent converges to $\max(-2^k, \min(2^k, x-y))$, and so its belief converges to the truth value of the predicate $x - y \geq 2^k$. Finally, this agent eventually meets all other agents, which change their beliefs to the same value.

It is shown in \cite{} that the protocol converges in $O(n^2 \log n)$ expected number of interactions. The number of 
states is however $\Omega(2^k)$, and so exponoential in the size of the predicate.


We obtain a protocol with a polynomial number of states by removing states and transitions from the protocol above.
More precisely, we retain exactly the states $(\ell, b, u)$ such that $u$ is a power of $2$, and the transitions which nly involve these states.


